ControversialQA: Exploring Controversy in Question Answering

Controversy is widespread online. Previous studies mainly define controversy based on vague assumptions of its relation to sentiment such as hate speech and offensive words. This paper introduces the first question-answering dataset that defines content controversy by user perception, i.e., votes from plenty of users. It contains nearly 10K questions, and each question has a best answer and a most controversial answer. Experimental results reveal that controversy detection in question answering is essential and challenging, and there is no strong correlation between controversy and sentiment tasks.

==> limitations.tex <==
The number of samples in ControversialQA is relatively small compared to the complex world. It may not cover all cases, especially since we only included data in English, ignoring the controversies in other languages. Meanwhile, controversy can be divided into finer-grained topics, such as gender or politics, which may require manual labeling from human annotators. Lastly, the controversy can also be expanded to other research directions besides QA in future research.
